Imaging results from the legacy GMRT Galaxy Cluster Key Project

We have used archival GMRT data to image and study 39 galaxy clusters. These observations were made as part of the GMRT Key Project on galaxy clusters between 2001 and 2004. The observations presented in this sample include 14 observations at 610 MHz, 29 at 325 MHz and 3 at 244 MHz covering a redshift range of 0.02 to 0.62. Multi-frequency observations were made for 8 clusters. We analysed the clusters using the SPAM processing software and detected the presence of radio halo emission for the first time in the clusters RXC J0510-0801 and RXC J2211.7-0349. We also confirmed the presence of extended emission in 11 clusters which were known from the literature. In clusters where halos were not detected upper limits were placed using our own semi-automated program. We plot our detections and non-detections on the empirical $L_X-P_{1.4}$ and $M_{500}-P_{1.4}$ relation in radio halo clusters and discuss the results. The best fits follow a power law of the form $L_{500} \propto P_{1.4}^{1.82}$ and $M_{500} \propto P_{1.4}^{3.001}$ which is in accordance with the best estimates in the literature.

==> Complete Manuscript/inputfigures.tex <==
\begin{figure*}
	\centering
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ1334_3+5031_618}
		\includegraphics[width=0.48\textwidth]{MCXCJ0505_3-2849_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ0505_3-2849_618}
		\includegraphics[width=0.48\textwidth]{MCXCJ1241_5+3250_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ1241_5+3250_618}
		\includegraphics[width=0.48\textwidth]{MCXCJ0256_5+0006_618}
		\subcaption{Radio images}
	 \end{subfigure}
	 \label{fig:images_1}
	 \caption{Radio images for the clusters in our sample. 
	 Dashed circles represents $R_{500}$ as given by MCXC.
	 The units of the colourbar are in Jansky/beam. 
	 These images were created using astropy with interval levels 
	 determined automatically for each image using the PercentileInterval option.
	 By default, 99\% of the pixels were used to estimate the limits with the exceptions 
	 being RXC J0847.1+3449 and RX J1046.8-2535 where 98\% of the pixels were used.}
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ0318_2-0301_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ0318_2-0301_618}
		\includegraphics[width=0.48\textwidth]{A2597_618}
		\includegraphics[width=0.48\textwidth]{MCXCJ0426_1+1655_240}
		\includegraphics[width=0.48\textwidth]{MCXCJ0426_1+1655_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ0426_1+1655_618}
		\caption{Radio images contd.}
	\end{subfigure}
	\label{fig:images_2}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ2237_0-1516_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ2237_0-1516_618}
		\includegraphics[width=0.48\textwidth]{A2319_618}
		\includegraphics[width=0.48\textwidth]{A2163_317}
		\includegraphics[width=0.48\textwidth]{A2163_618}
		\includegraphics[width=0.48\textwidth]{A2345_618}
		\caption{Radio images contd.}
\end{subfigure}
\label{fig:images_3}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ1701_3+6414_333}
		\includegraphics[width=0.48\textwidth]{A2390_240}
		\includegraphics[width=0.48\textwidth]{A665_240}
		\includegraphics[width=0.48\textwidth]{MCXCJ1308_5+5342_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ1308_5+5342_618}
		\includegraphics[width=0.48\textwidth]{MCXCJ0847_1+3449_333}
		\caption{Radio images contd.}
\end{subfigure}
\label{fig:images_4}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ0847_1+3449_618}
		\includegraphics[width=0.48\textwidth]{A0400_333}
		\includegraphics[width=0.48\textwidth]{MCXCJ1120_1+4318_334}
		\includegraphics[width=0.48\textwidth]{A1084_317}
		\includegraphics[width=0.48\textwidth]{MCXCJ2211_7-0349_317}
		\includegraphics[width=0.48\textwidth]{A0545_317}
		\caption{Radio images contd.}
\end{subfigure}
\label{fig:images_5}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{A1689_317}
		\includegraphics[width=0.48\textwidth]{A0901_317}
		\includegraphics[width=0.48\textwidth]{A0291_317}
		\includegraphics[width=0.48\textwidth]{MCXCJ1212_3-1816_317}
		\includegraphics[width=0.48\textwidth]{1046-25_GMRT325_SP2B_PBCOR_FITS_317}
		\includegraphics[width=0.48\textwidth]{A2104_317}
		\caption{Radio images contd. Note that no $R_{500}$ circle is shown for RXJ1046.8-2535
		since no X-ray information is available for that cluster.}
\end{subfigure}
\label{fig:images_6}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{MCXCJ0510_7-0801_317}
		\includegraphics[width=0.48\textwidth]{AS0780_317}
		\includegraphics[width=0.48\textwidth]{A2485_317}
		\includegraphics[width=0.48\textwidth]{MCXCJ0437_1+0043_317}
		\includegraphics[width=0.48\textwidth]{A0907_317}
		\includegraphics[width=0.48\textwidth]{A3444_317}
		\caption{Radio images contd.}
\end{subfigure}
\label{fig:images_7}	
\end{figure*}

\begin{figure*}\ContinuedFloat
	\begin{subfigure}{\textwidth}
		\includegraphics[width=0.48\textwidth]{A1300_317}
		\includegraphics[width=0.48\textwidth]{MCXCJ1504_1-0248_317}
		\includegraphics[width=0.48\textwidth]{MCXCJ1514_9-1523_317}
		\includegraphics[width=0.48\textwidth]{A2537_317}
		\caption{Radio images contd.}
\end{subfigure}
\label{fig:images_8}	
\end{figure*}


